A stochastic approach to the reconstruction of spectral functions in lattice QCD

We present a Stochastic Optimization Method (SOM) for the reconstruction of the spectral functions (SPFs) from Euclidean correlation functions. In this approach the SPF is parameterized as a sum of randomly distributed boxes. By varying the width, location and height of the boxes stochastically an optimal SPF can be obtained. Using this approach we reproduce mock SPFs fairly well, which contain sharp resonance peaks, transport peaks and continuum spectra. We also analyzed the charmonium correlators obtained from $N_{\tau}$=96, 48, 32 lattices using SOM and found similar conclusion on the dissociation temperatures of charmonium ground states as that obtained using the Maximum Entropy Method.

==> pics/notes <==
\begin{figure}[h]
\begin{minipage}[b]{0.5\textwidth} 
	\centering
    \includegraphics[width=\textwidth]{pics/realdata_som.pdf}
	\caption{SPFs of charmonium in Vector channels at different temperatures.}
	\label{realdata}
\end{minipage}%
\begin{minipage}[b]{0.495\textwidth}
\centering
	\begin{tabular}{|c|ccc|}
		\hline
		 & $0.73T_c$ & $1.46T_c$ & $2.20T_c$ \\ \hline
		$SOM$ & $3.44$ & $4.8$ & $4.1$ \\ \hline
		$MEM$ & $3.48$ & $4.7$ & $??$\\ \hline
	\end{tabular}
	\caption{Peak-locations in [GeV] from SOM and MEM. }
	\label{tab_compare_som_mem}
\end{minipage}
\end{figure}



==> pics/notes_ <==
\begin{figure}[h]
\begin{minipage}[b]{0.5\textwidth} 
	\centering
    \includegraphics[width=0.8\textwidth]{pics/realdata_som.pdf}
	\caption{ \textit{Left}: Intercept is set to be 0.32. The small figure inside is the same as the outside one but in a small $\tilde{\omega}$ range to show the intercept clearly.   \textit{Right}: Intercept is increased to 1.32.}
	\label{realdata}
\end{minipage}%
\begin{minipage}[b]{0.5\textwidth}
\centering
	\begin{tabular}{|c|ccc|}
		\hline
		$T$ & $1.1T_c$ & $1.2T_c$ & $1.4T_c$ \\ \hline
		$\left(\frac{\sigma}{C_{em}T}\right)_{max}$ & $0.436$ & $0.365$ & $0.361$ \\ 
		$\left(\frac{\sigma}{C_{em}T}\right)_{min}$ & $0.217$ & $0.211$ & $0.217$\\ \hline
	\end{tabular}
	\tabcaption{Final results for the electrical conductivity. Note that the 
		systematic error from the cut-procedure and the statistical fit
	error are included (see text).}
	\label{tab_sigma_res}
\end{minipage}
\end{figure}


